Couplings for Multinomial Hamiltonian Monte Carlo

Hamiltonian Monte Carlo (HMC) is a popular sampling method in Bayesian inference. Recently, Heng & Jacob (2019) studied Metropolis HMC with couplings for unbiased Monte Carlo estimation, establishing a generic parallelizable scheme for HMC. However, in practice a different HMC method, multinomial HMC, is considered as the go-to method, e.g. as part of the no-U-turn sampler. In multinomial HMC, proposed states are not limited to end-points as in Metropolis HMC; instead points along the entire trajectory can be proposed. In this paper, we establish couplings for multinomial HMC, based on optimal transport for multinomial sampling in its transition. We prove an upper bound for the meeting time - the time it takes for the coupled chains to meet - based on the notion of local contractivity. We evaluate our methods using three targets: 1,000 dimensional Gaussians, logistic regression and log-Gaussian Cox point processes. Compared to Heng & Jacob (2019), coupled multinomial HMC generally attains a smaller meeting time, and is more robust to choices of step sizes and trajectory lengths, which allows re-use of existing adaptation methods for HMC. These improvements together paves the way for a wider and more practical use of coupled HMC methods.

==> pairing.tex <==
\subsection{Pairing-based coupling}

Finally, we describe a cheaper alternative that shares the same motivation as the OT-based coupling, and also draw a link to combinatorial optimization.
Instead of finding the joint $\gamma$ directly as in \eqref{eq:OT-objective},
we first decompose $\gamma = \mathbf{M} \mathbf{p}^\top$ and then solve \eqref{eq:OT-objective} w.r.t. $\mathbf{M}$,
where $\mathbf{M}$ represents the conditional probability of $j$ given $i$ and $\mathbf{p}$ is the probability vector of the categorical distribution $p$.
We can further restrict $\mathbf{M} \in \{0, 1\}^{K \times K}$, i.e. a deterministic \textit{pairing} from $i$ to $j$, 
and the optimization problem becomes the well-known \textit{assignment problem} \citep{burkard2012assignment}. %
Although the algorithmic complexity of exact algorithms for this problem is also $\mathcal{O}(K^3)$,
exact exacting solvers and approximate solvers tends be faster than those for OT.
For simplicity,
we will solve the assignment problem using the Hungarian algorithm \citep{kuhn_hungarian_1955}.
Assuming we have obtained the pairing matrix $\mathbf{M}$,
simply sampling from the joint $\mathbf{M} \mathbf{p}^\top$ will lead to biased samples from the coupled kernel since the marginals are not preserved.

To this end, we introduce Algorithm~\ref{alg:pairing} to sample indices that retains the marginals once obtaining such a pairing matrix $\mathbf{M}$,
which is inspired by the maximal coupling method \citep{thorisson_coupling_2000},
\begin{algorithm}
    \SetAlgoLined
    \textbf{Input}: two probability vectors $\mathbf{p}$ and $\mathbf{q}$ of length $K$ and pair-wise distance matrix $\mathbf{D}$\;
    \textbf{Output}: indices $(i, j)$ from a coupling of $\Cat(\mathbf{p})$ and $\Cat(\mathbf{q})$\;
    Compute the conditional matrix $\mathbf{M}$ by solving \eqref{eq:OT-objective} with $\gamma = \mathbf{M} \mathbf{p}^\top$\;
    Compute the paired probability vector $\mathbf{r} = \mathbf{M} \mathbf{p}$\;
    Compute the probability of pairing $w^\ast = \min_j q_j / r_j$\; 
    Sample $i \sim \Cat(\mathbf{p})$\;
    Sample $u \sim \mathcal{U}(0, 1)$\;
    \eIf{$u < w^\ast$}{
        Sample $j \sim \Cat(\mathbf{m}_i)$, where $\mathbf{m}_i$ is the $i$-th column of $\mathbf{M}$\;
        Output $(i, j)$\;
    }{
        Compute the debiasing probability vector $\mathbf{t} = (\mathbf{q} - \mathbf{r} w^\ast) / (1 - w^\ast)$\;
        Sample $j \sim \Cat(\mathbf{t})$\;
        Output $(i, j)$\;
    }
    \caption{Intra-trajectory coupling with pairing}
    \label{alg:pairing}
\end{algorithm}

Note that even though we have considered $\mathbf{M}$ to be a binary matrix,
Algorithm~\ref{alg:pairing} is more generic: $\mathbf{M}$ can be any conditional distribution of $j$ given $i$.
Therefore,
even if the solution of $\mathbf{M}$ is approximate,
it will still preserve the marginals because of the debiasing step.
Therefore, one can also apply Algorithm~\ref{alg:pairing} with a approximate solution $\hat{\gamma}$ from \eqref{eq:OT-objective} and replace Line 3 to compute the joint $\mathbf{M}$ from joint $\hat{\gamma}$ as ``compute $\mathbf{M} = \hat{\gamma} \oslash (\mathbf{1}^\top \hat{\gamma})$',
where $\oslash$ represents the Hadamard division.

\paragraph{Algorithm~\ref{alg:pairing} yields $i \sim p$ and $j \sim q$}
We now verify Algorithm~\ref{alg:pairing} leaves the marginals unchanged. 
First notice that Line 5 indicates $i \sim p$.
To find the marginal distribution of $j$, we write 
\begin{equation}
    \begin{aligned}
        P(j = j') 
        &= P(j = j'| C_1) P(C_1) + P(j = j'| C_2) P(C_2) \\
        &= \left(\sum_i M_{j',i} p_i \right) w^\ast + t_{j'} (1 - w^\ast) = r_{j'} w^\ast + \frac{q_{j'} - r_{j'} w^\ast}{1 - w^\ast} (1 - w^\ast) = q_{j'}
    \end{aligned},
    \label{eq:pairing-proof}
\end{equation}
where $C_1$ and $C_2$ are events of entering the first and second branches in Line 8 and Line 11 respectively, $M_{j',i}$ is $j'$-th row, $i$-th column entry of $\mathbf{M}$ and $p_i$, $q_j$ are the $i$-th entry of $\mathbf{p}$ and $j$-th entry of $\mathbf{q}$ respectively.
As a result of \eqref{eq:pairing-proof}, $j \sim q$.
Notice that Line 4 ensures the numerator in the RHS of Line 12 has no negative entries and therefore $\mathbf{t}$ is a valid probability vector.
Also notice that $w^* \leq 1$, so that the denominator of $\mathbf{t}$ is positive. This follows from the fact that $w^* = \min_j q_j / r_j$, and that $\mathbf{q}$ and $\mathbf{r}$ are both probability vectors.







==> plots/proof/combined.tex <==
\begin{tikzpicture}[fill=gray]
    \scope
    \clip 
        (-2,-2.5) rectangle (2,2.5) 
        (0,-1.25) ellipse (0.75 and 1.25);
    \fill[opacity=0.5] (-2,-2.5) rectangle (2,2.5);
    \endscope
    \scope
    \clip 
        (-2,-2.5) rectangle (2,2.5)
        (0,0) ellipse (2 and 1);
    \fill[opacity=0.5] (0,-1.25) ellipse (0.75 and 1.25);
    \endscope
    \draw 
        (0,0) circle (2) 
            (0,2) node [text=black,below] {$ S \times S $}
        (0,0) ellipse (2 and 1) 
            (0,0) node [text=black,above] {$ L_{\ell_0}(U_S) \times L_{\ell_0}(U_S) $}
        (0,-1.25) ellipse (0.75 and 1.25) 
            (0,-0.5) node [text=black] {$ \bar{C}_\delta $}
        (0,-1.25) ellipse (0.75 and 1.25) 
            (0,-1.25) node [text=black] {$ D_\delta $}
        (-2,-2.5) rectangle (2,2.5) 
            (1.25,2.5) node [text=black,below] {$ \RR^d \times \RR^d $};
\end{tikzpicture}

==> plots/proof/global_lyapunov_function.tex <==
\begin{tikzpicture}[fill=gray]
    \scope
    \clip 
        (-2,-2.5) rectangle (2,2.5) 
        (0,0) ellipse (2 and 1);
    \fill[opacity=0.5] (-2,-2.5) rectangle (2,2.5);
    \endscope
    \draw 
        (0,0) circle (2) 
            (0,2) node [text=black,below] {$ S \times S $}
        (0,0) ellipse (2 and 1) 
            (0,0) node [text=black] {$ L_{\ell_0}(U_S) \times L_{\ell_0}(U_S) $}
        (-2,-2.5) rectangle (2,2.5) 
            (1.25,2.5) node [text=black,below] {$ \RR^d \times \RR^d $};
\end{tikzpicture}

==> plots/proof/local_contractivity.tex <==
\begin{tikzpicture}[fill=gray]
    \scope
    \clip 
        (-2,-2.5) rectangle (2,2.5) 
        (0,-1.25) ellipse (0.75 and 1.25);
    \fill[opacity=0.5] (0,0) circle (2);
    \endscope
    \draw 
        (0,0) circle (2) 
            (0,2) node [text=black,below] {$ S \times S $}
        (0,-1.25) ellipse (0.75 and 1.25) 
            (0,-1.25) node [text=black] {$ D_\delta $}
        (-2,-2.5) rectangle (2,2.5) 
            (1.25,2.5) node [text=black,below] {$ \RR^d \times \RR^d $};
\end{tikzpicture}

==> theoretical.tex <==
\section{Theoretical analysis}
\label{sec:theoretical}

\cs{If this subsection gets long, we can promote it to a top-level section.}

\tor{Maybe everything but the results can just be put into the appendix, and we replace this entire section with "Theoretical results" where we just list the assumptions and then include the content in the current "Results" section? We can simply refer the reader to \citet{heng_unbiased_2019} for the understanding of what's going on with the lemmas and whatnot.}

The goal of this section is to establish that MC-HMC indeed satisfies the assumptions outlined in Section \ref{sec:unbiased-MCMC}. To that end, following \citet{heng_unbiased_2019}, we make the following assumptions on the potential function $U$.

\begin{assumption}[Regularity and growth of potential]\label{assumpt:regularity-and-growth-of-potential}
  The potential $U$ is twice continuously differentiable and its gradient $\nabla U: \mathbb{R}^d \to \mathbb{R}^d$ is globally $\beta \text{-Lipschitz}$, i.e. $\exists \beta > 0$ such that
  \begin{equation*}
    \sqeuclid{\nabla U(q) - \nabla U(q')} \le \beta \sqeuclid{q - q'}, \quad \forall q, q' \in \mathbb{R}^d
  \end{equation*}
\end{assumption}

\begin{assumption}[Local strong convexity of potential]\label{assumpt:strong-convexity-potential}
  There exists a compact set $S \in \mathcal{B}(\mathbb{R}^d)$ with positive Lebesgue measure, such that the restriction of $U$ to $S$ is $\alpha \text{-strongly}$ convex. That is,
\begin{equation*}
(q - q')^T \big( \nabla U(q) - \nabla U(q') \big) \ge \alpha \sqeuclid{q - q'}^2, \quad \forall, q, q' \in S
\end{equation*}
\end{assumption}

\todo{Mention uniqueness due to \assumptref{assumpt:regularity-and-growth-of-potential}. Not sure why they're being explicit about uniqueness globally on $\mathbb{R}_{ + }$ in \citet{heng_unbiased_2019}. Seems like we only need uniqueness on some set around current point, e.g. $[-T, T]$ for some $T > 0$. This also makes things easier for us.}

Note that due to the equations for the Hamiltonian system in Eq.~\eqref{eq:hamiltonian-flow}, this is in fact an assumption on the evolution of the momenta of the system. It implies at most quadratic growth of the potential, or equivalently that the tails of the target distribution are no lighter than Gaussian \citep{heng_unbiased_2019}.

Note that \assumptref{assumpt:strong-convexity-potential} is equivalent to assuming that the target distribution $\pi$ is strongly log-concave often seen in the MCMC literature \todo{refs}. In our case it is more convenient to work with the potential directly. 


\tor{Maybe start the section off by saying something along the lines of "In this section we closely follow \citet{heng_unbiased_2019}" so we don't have to repeatedly say "following \citet{heng_unbiased_2019}" etc.}

As shown by \citet{heng_unbiased_2019}, making use of the equations for the Hamiltonian system in \secref{sec:hamiltonian-flows}, we have
\begin{equation}
    \frac{1}{2} \dv{t} \sqeuclid{\Delta(t)}^2 = \Delta(t)^T \big( p^1(t) - p^2(t) \big)
\end{equation}
where $\Delta(t) := \sqeuclid{q^1(t) - q^2(t)}$. This is the main motivation behind sharing the momentum as in \algref{alg:hmc-coupling} -- when $p^1(0) = p^2(0)$ we observe that at $t = 0$ we have $\dv{t} \sqeuclid{\Delta(t)}^2 = 0$, i.e. a local optima. To ensure that this is in fact a strict local \emph{maximum}, we make use of \assumptref{assumpt:strong-convexity-potential} which then gives
\begin{equation*}
    \frac{1}{2} \dv[2]{t} \sqeuclid{\Delta(t)}^2 \le - \alpha \sqeuclid{\Delta(0)}^2
\end{equation*}
for some $\alpha > 0$ and with $q_0^1, q_0^2 \in S$ with $q_0^1 \ne q_0^2$. In conclusion, by sharing the momentum and assuming \assumptref{assumpt:strong-convexity-potential}, we can ensure that simulating the flow for some time $t \in [-T, T] \setminus \set{0}$ will decrease the distance between the points on the trajectory. In fact, because of continuity of $t \mapsto \sqeuclid{\Delta(t)}^2$, we can obtain the following lemma.

\begin{lemma}[{\citep[Lemma 1]{heng_unbiased_2019} slightly modified}]\label{lemma:lemma1-heng}
  Suppose that the potential $U$ satisfies Assumptions \ref{assumpt:regularity-and-growth-of-potential} and \ref{assumpt:strong-convexity-potential}. For any compact set $A \subset S \times S \times \mathbb{R}^d$, where $S$ is as in \assumptref{assumpt:strong-convexity-potential}, there exists a trajectory length $T > 0$ such that for any $t \in [-T, T] \setminus \set{0}$ there exists $\rho \in [0, 1)$ such that
  \begin{equation}
      \sqeuclid{\flowq{t}(q_0^1, p_0) - \flowq{t}(q_0^2, p_0)} \le \rho \sqeuclid{q_0^1 - q_0^2}, \quad \forall (q_0^1, q_0^2, p_0) \in A
  \end{equation}
\end{lemma}

\subsection{Results}
As mentioned before, the main difference between our work and the work of~\cite{heng_unbiased_2019} is that our method makes use of multinomial sampling instead of a Metropolis-Hastings step. As a result, for MC-HMC with quantile coupling we are able to inherit the main results of~\cite{heng_unbiased_2019} with a small amount of work. Of particular importance are the following theorems which tells us that under certain conditions our method satisfies \assumptref{assumpt:tail-of-meeting-time}.

\tor{Maybe just move this theorem to the appendix? The important theorem is Thm 2}
\begin{theorem}[\cite{heng_unbiased_2019} simplified]\label{thm:geometric-tailed-meeting-time-HMC-simplified}
  Suppose $U$ satisfies Assumptions~\ref{assumpt:regularity-and-growth-of-potential} and~\ref{assumpt:strong-convexity-potential}. Under some additional assumptions (see appendix), we then have that there exists $\stepsize{} > 0$ and $L \in \mathbb{N}$ such that
  \begin{equation*}
    \PkerHMC{\stepsize{}}{L}(\tau_{\delta} > n) \le C_0 \kappa_0^n
  \end{equation*}
  for some $C_0 \in \mathbb{R}_{ + }$ and $\kappa_0 \in (0, 1)$ and for all integers $n \ge 0$.
\end{theorem}


Theorem~\ref{thm:geometric-tailed-meeting-time-HMC-simplified} states that under certain assumptions the distribution over the \emph{relaxed} $\tau_{\delta}$ meeting time for the HMC kernel with quantile coupling decreases geometrically.

\begin{theorem}[\cite{heng_unbiased_2019} simplified]\label{thm:geometric-tailed-meeting-time-simplified}
  Suppose that $U$ satisfies Assumptions~\ref{assumpt:regularity-and-growth-of-potential} and~\ref{assumpt:strong-convexity-potential}. Under some additional assumptions (see appendix), we then have that there exists $\stepsize{} > 0$, $L \in \mathbb{N}$ and $\sigma > 0$ such that
  \begin{equation}
    \Pker{\stepsize{}}{L}{\sigma}(\tau > n) \le C_0 \kappa_0^n
  \end{equation}
  for some $C_0 \in \mathbb{R}_{ + }$ and $\kappa_0 \in (0, 1)$ and for all integers $n \ge 0$.
\end{theorem}

Theorem~\ref{thm:geometric-tailed-meeting-time-simplified} states that under certain assumptions the distribution over the meeting time $\tau$ for the mixture kernel with an HMC component with quantile coupling decreases geometrically.

To ensure that these results from~\cite{heng_unbiased_2019} apply to MC-HMC with quantile coupling it turns out that we only need to prove the following statement:

\begin{lemma}[\cite{heng_unbiased_2019}, S5]\label{lemma:statement-5-multinomial}
  Assume that $U$ satisfies Assumptions~\ref{assumpt:regularity-and-growth-of-potential} and~\ref{assumpt:strong-convexity-potential}.
  Moreover let $A := S \times S \times K^{-1}([0, k_0])$ and suppose that the chains $\big( Q_n^1 \big)_{n \ge 0}$ and $\big( Q_n^2 \big)_{n \ge 0}$ are initialized at $Q_0^1 = q^1 \in S$ and $Q_0^2 = q^2 \in S$, respectively.
  
  Then there exist $\rho_1 \in (0, 1)$, $\omega_1 \in (0, 1)$ and $\omega_2 \in (0, \omega_1)$ such that
  for all $(Q_0^1, Q_0^2, P_1) \in S \times S \times K^{-1}([0, k_0])$.
\end{lemma}

Lemma~\ref{lemma:statement-5-multinomial} essentially states that when we reach this set $S$, there is a non-zero probability of decreasing the distance between the two chains as we sample from the coupled HMC kernel with shared momentum. Once this has been established, one can follow \citet{heng_unbiased_2019} to prove that the maximal coupling within the coupled RWMH kernel $\KerCMH_{\sigma}$ proposes the same value for both chains with a probability arbitrarily close to 1 and thus Theorem~\ref{thm:geometric-tailed-meeting-time-simplified}.
With some modifications to the proof of Proposition 1 in~\cite{heng_unbiased_2019}, it is quite straight-forward to prove that Lemma~\ref{lemma:statement-5-multinomial} holds for the quantile coupling. The idea behind the proof is that as we make the integrator sufficiently accurate, the marginal distributions over elements in the respective trajectories becomes uniform. The quantile coupling then converges to a diagonal coupling, thus making the probability of sampling indices $(k^1, k^2) \sim \gamma$ such that $k^1 = k^2 = k$ for some $k \ne 0$ can be made sufficiently large. Then employing Lemma~\ref{lemma:lemma1-heng} we can convert this into a non-zero lower bound on the probability of the proposed positions decreasing in distance compared to the current positions, as wanted.

Finally, since the only difference between MC-HMC with quantile coupling $\gamma$ and optimal transport coupling $\gamma^{ * }$ is the choice of indices $(k^1, k^2)$ for the trajectories, it is sufficient to ensure that $\gamma_{k^1 k^2}^{ * } > 0$ for all $(k^1, k^2)$ such that $\gamma_{k^1, k^2} > 0$. This can easily be done by forcing $\gamma^{ * }$ to have non-zero probability mass everywhere, which we can do since both the marginals will always have non-zero probability mass everywhere. That is, we just replace the non-negative constraints $\gamma_{ij} \ge 0$ in Eq.~\eqref{eq:OT-objective} with positive constraints $\gamma_{ij} > 0$, and we are done. Alternatively, one can use a mixture of the optimal transport coupling and the quantile coupling to ensure the same property. This also works for proving that the pairing coupling satisfies Lemma~\ref{lemma:statement-5-multinomial}.

The full proof can be found in the appendix.

\subsection{Theoretical results: take 2}
To ensure that these results from \citet{heng_unbiased_2019} apply to MC-HMC with maximal coupling, it turns out that it is sufficient to prove the following statement:

\begin{lemma}
Assume that $U$ satisfies Assumptions~\ref{assumpt:regularity-and-growth-of-potential} and~\ref{assumpt:strong-convexity-potential}.

For any $k_0 > 0$ there exists $\stepsize > 0$, $L \in \mathbb{N}$, $\rho_1 \in (0, 1)$, $\omega_1 \in (0, 1)$ and $\omega_2 \in (0, \omega_1)$ such that
\begin{equation*}
\PkerHMC{\stepsize{}}{L} \Bigg( \bigcup_{l \ne 0} \left\{ \left| \flowdisc{\stepsize{}}{l}(Q_0^1, P_1^*) - \flowdisc{\stepsize{}}{l}(Q_0^2, P_1^*) \right| \le \rho_1 \left| Q_0^1 - Q_0^2 \right| \right\} \Bigg) \ge \omega_1
\end{equation*}
and
\begin{equation*}
\PkerHMC{\stepsize{}}{L} \Big( \left\{ l_1 = l_2 \ne 0 \right\} \Big) \ge 1 - \omega_2
\end{equation*}
for all $\big( Q_0^1, Q_0^2, P_1^{ * } \big) \in S \times S \times K^{-1}([0, k_0])$.
\end{lemma}





==> theoretical_new.tex <==
We now establish geometric tails for the relaxed meeting time for the proposed coupled HMC kernels. %
Following a similar argument in \citet{heng_unbiased_2019}, such coupled HMC kernels can be used together with coupled RWMH kernel in a mixture manner to trigger exact meeting, thus satisfying \assumptref{ass:tail_of_meeting_time} and \ref{ass:faithfullness}.

Following \citet{heng_unbiased_2019},
we make two assumptions on the potential function $U: \RR^d \mapsto \RR $. %
\begin{assumption}[Regularity and growth of potential]
  The potential $U$ is twice continuously differentiable and its gradient $\nabla U: \RR^d \mapsto \RR^d$ is globally $\beta$-Lipschitz, i.e. there exists $\beta > 0$ such that
  $\norm{\nabla U(q) - \nabla U(q')} \leq \beta \norm{q - q'}$
  for all $q, q' \in \RR^d$.
  \label{ass:regularity_and_growth}
\end{assumption}
\begin{assumption}[Local strong convexity of potential]
  There exists a compact set $S \in \calB(\RR^d)$, with positive Lebesgue measure, s.t. the restriction of the potential $U$ to $S$ is $\alpha$-strongly convex, i.e.,
  $\exists\;\alpha > 0$ s.t. $(q - q')^\top \left( \nabla U(q) - \nabla U(q') \right) \geq \alpha \norm{q - q'}^2$
  for all $q, q' \in S$.
  \label{ass:local_strong_convexity}
\end{assumption}

\paragraph{Proof sketch}
Despite the similarity in assumptions, our proof strategy is somewhat different from \citep{heng_unbiased_2019}.
Since \citet{heng_unbiased_2019} are working with a Metropolis HMC kernel, they take an approach heavily inspired from their previous work on coupled Metropolis-Hastings type kernels \citep{jacob_unbiased_2019}. 
Here, on the other hand, we are working with multinomial HMC and thus the approach does not translate directly. We introduce a new proof strategy, taking inspiration from \citet{heng_unbiased_2019} where suitable, that consists the following two stages.
In the \underline{first stage} (see \secref{sec:theory-local_contractivity}), we establish, under similar conditions as \citet{heng_unbiased_2019}, our method with maximal coupling \textit{contracts locally}; i.e. the \emph{expected} distance reduces after each transition in some local regions. And the fact that maximal coupling contracts locally immediately implies that the OT coupling also contract locally, since the OT coupling by definition obtains the minimum expected distance, with the expectation taken over the indices of the trajectory.
In the \underline{second stage} (\secref{sec:theory-tails}), we show that local contractivity combined with an additional assumption on the existence of a global Lyapunov function, lead to geometric tails for the relaxed meeting time $ \tau_\delta = \inf \{ n \geq 0 : (X_n, Y_{n-1}) \in D_\delta \} $ where $ D_\delta := \{ (X, Y) : \norm{X - Y} \leq \delta \} $ for any $\delta > 0$.
This is done by constructing a combined Lyapunov function that controls excursions outside of a set $\bar{C}_\delta \subseteq D_\delta$.

\subsection{Local contractivity}
\label{sec:theory-local_contractivity}

The goal of this section is to establish local contractivity for coupled multinomial HMC kernels with maximal coupling $\gamma^\ast$ and OT coupling $\gamma^\circ$.
\begin{definition}[Contractivity]
    For a compact set $\bar{S} \subset \calB(\RR^d) \times \calB(\RR^d)$,
    we say a coupled kernel $\CMKer$ is \textit{contractive} or \textit{has the contractivity property} on $\bar{S}$ if and only if there exists $\lambda_0 \in (0, 1) $ satisfying
    \begin{equation*}
        \E[\CMKer]{ \norm{x' - y'} \mid x, y } \leq \lambda_0 \norm{x - y}
        \label{eq:contractivity}
    \end{equation*}
    for all $(x, y) \in \bar{S}$,
    where $\lambda_0$ is called the \textit{contractivity rate}.
    When $\bar{S} = S \times S$ where $S$ is from \assumptref{ass:local_strong_convexity},
    we refer such contractivity as \textit{local contractivity} and call the kernel \textit{locally contractive}.
\end{definition}

To assist the proof, 
we introduce a family of joint distributions called the \textit{parallel-in-time joint}, $J^\parallel$,
which is a joint distribution that consists diagonal entries only.
$J^\parallel$ is closely related to $\gamma^\ast$ via the total variation distance.
We will first establish a useful property of $J^\parallel$ (\secref{sec:theory-local_contractivity-parallel}).
We will then exploit the property of $J^\parallel$ to show local contractivity for $\gamma^\ast$
by controlling the numerical errors in the leapfrog integration (\secref{sec:theory-local_contractivity-maximal}).
Finally we show $\gamma^\circ$ is contractive by noting that the the local contractivity rate for $\gamma^\circ$ is at least as small as for $\gamma^\star$, hence $\gamma^\circ$ is contractive by contractivity of $\gamma^\star$ (\secref{sec:theory-local_contractivity-ot}).

\subsubsection{Parallel-in-time joint}
\label{sec:theory-local_contractivity-parallel}

To establish a useful property of $J^\parallel$,
we first introduce the following lemma.

\begin{lemma}
    Suppose that the potential $U$ satisfies Assumptions \ref{ass:regularity_and_growth} and \ref{ass:local_strong_convexity}. For any compact set $A \subset S \times S \times \mathbb{R}^d$, there exists a trajectory length $T > 0$ and a step size $\stepsize{}_1 > 0 $ s.t. for any $\stepsize{} \in (0, \stepsize{}_1]$ and any $t \in [-T, T] \setminus \set{0}$ with $l := t / \stepsize{} \in \ZZ$,
    there exists $\rho \in [0, 1)$ satisfying
    \begin{equation}
        \norm{\flowqdisc{\stepsize{}}{l}(q_0^1, p_0) - \flowqdisc{\stepsize{}}{l}(q_0^2, p_0)} \leq \rho \norm{q_0^1 - q_0^2}
        \label{eq:local_abs_contractivity}
    \end{equation}
    for all $(q_0^1, q_0^2, p_0) \in A$.
    \label{lemma:local_abs_contractivity}
\end{lemma}
\begin{proof}
    The proof is done by combining properties of leapfrog integrators and Lemma 1 in \citet{heng_unbiased_2019}.
    See Appendix~\ref{app:proof-local_abs_contractivity}.
\end{proof}
Lemma~\ref{lemma:local_abs_contractivity} can be viewed as an unadjusted numerical version of Lemma 1 in \citet{heng_unbiased_2019} that generalizes to both forward and backward simulations.

Proposition~\ref{prop:property-parallel} summarizes a useful property of $J^\parallel$ as a direct result of applying Lemma~\ref{lemma:local_abs_contractivity}.
\begin{proposition}
    Suppose that $U$ satisfies Assumptions \ref{ass:regularity_and_growth} and \ref{ass:local_strong_convexity}.
    For any compact set $A \subset S \times S \times \mathbb{R}^d$ and any parallel-in-time joint $J^\parallel \in \RR^{K \times K}$, 
    there exists a trajectory length $T > 0$, a step size $\stepsize{}_1 > 0 $ s.t. for any $\stepsize{} \in (0, \stepsize{}_1]$ and any $L_1, L_2 \in \NN$ with $L_1 + L_2 = K - 1$ and $\stepsize{} L_1, \stepsize{} L_2 < T$,
    there exists $\lambda_1 \in (0, 1)$ satisfying
    \begin{equation}
        \E[(i, j) \sim J^\parallel] { \norm{\flowqdisc{\stepsize{}}{l_i}(q_0^1, p_0) - \flowqdisc{\stepsize{}}{l_j}(q_0^2, p_0)} } \leq \lambda_1 \norm{q_0^1 - q_0^2}
        \label{eq:property-parallel}
    \end{equation}
    for all $(q_0^1, q_0^2, p_0) \in A$,
    where $l_k$ is the $k$-th entry of the vector $[-L_1, \dots, 0, \dots, L_2]$.
    \label{prop:property-parallel}
\end{proposition}

\begin{proof}
    A direct result of Lemma~\ref{lemma:local_abs_contractivity}.
    See Appendix~\ref{app:proof-property-parallel}.
\end{proof}

\subsubsection{Maximal coupling}
\label{sec:theory-local_contractivity-maximal}

To establish local contractivity for coupled multinomial HMC with $\gamma^\ast$,
we first introduce a proposition on the total variation distance between $\vp$ and $\vq$.
\begin{proposition}
    Suppose that $U$ satisfies Assumptions \ref{ass:regularity_and_growth} and \ref{ass:local_strong_convexity}.
    For any Hamiltonian trajectory of length $T$ with $L$ discretization steps and $(i, j) \sim \gamma^\ast $, 
    we have for any $\delta > 0$, there exists $\stepsize{}_2 > 0$ s.t. for any $\stepsize{} \in (0, \stepsize{}_1]$
    \begin{equation}
        \TV( \vp, \vq ) = \PP(i \neq j) < \delta.
    \end{equation}
    In words, the probability mass put on the diagonal of $\gamma^\star$ can be made arbitrarily close to 1 by increasing the number of discretization steps.
    \label{prop:maximal_coupling}
\end{proposition}
\begin{proof}
    The proof uses the 1-Lipschitz property of the softmax function \citep{gao2018properties} in \eqref{eq:multi-intra} to bound the probability differences introduced by numerical errors.
    See Appendix~\ref{app:proof-maximal_coupling}.
\end{proof}
With Proposition~\ref{prop:maximal_coupling}, 
we can establish the local contractivity for our coupled HMC kernel with the maximal coupling $\gamma^\ast$.
\begin{lemma}
    Suppose that the potential $U$ satisfies Assumptions \ref{ass:regularity_and_growth} and \ref{ass:local_strong_convexity}.
    For a maximal coupling $\gamma^\ast$, 
    there exists a trajectory length $T > 0$ and a step size $\stepsize{}_2 > 0 $ such that for any $\stepsize{} \in (0, \min\{\stepsize{}_1, \stepsize{}_2\}]$ and any $t \in [-T, T] \setminus \set{0}$ with $l := t / \stepsize{} \in \ZZ$,
    there exists $\lambda_2 \in (0, 1)$ satisfying
    \begin{equation}
        \E[\CMKer_{\stepsize, l}^\ast]{ \norm{q^1 - q^2} \mid q_0^1, q_0^2} \leq \lambda_2 \norm{q_0^1 - q_0^2}
        \label{eq:contractivity-maximal}
    \end{equation}
    for all $(q_0^1, q_0^2) \in S \times S$,
    where $\CMKer_{\stepsize, l}^\ast$ is the coupled kernel in Algorithm~\ref{alg:coupled-hmc} with (i) shared momentum, (ii) shared forward and backward simulation steps and (iii) $(i, j) \sim \gamma^\ast$ for intra-trajectory sampling.
    \label{lemma:contractivity-maximal}
\end{lemma}

\begin{proof}
    With Proposition~\ref{prop:maximal_coupling}, for a given integration time, we are allow to choose step size arbitrary small to increase probability of picking parallel-in-time pairs, whose contractivity is established in Proposition~\ref{prop:property-parallel}.
    See Appendix~\ref{app:proof-contractivity-maximal} for the complete proof.
\end{proof}

\subsubsection{OT coupling}
\label{sec:theory-local_contractivity-ot}
By the definition of OT coupling in \eqref{eq:ot_objective} and Lemma~\ref{lemma:contractivity-maximal}, we have the following result.
\begin{lemma}
    Suppose that the potential $U$ satisfies Assumptions \ref{ass:regularity_and_growth} and \ref{ass:local_strong_convexity}.
    For any OT $\gamma^\circ$, 
    there exists a trajectory length $T > 0$ and a step size $\stepsize{}_2 > 0 $ such that for any $\stepsize{} \in (0, \min\{\stepsize{}_1, \stepsize{}_2\}]$ and any $t \in [-T, T] \setminus \set{0}$ with $l := t / \stepsize{} \in \ZZ$,
    there exists $\lambda_2 \in (0, 1)$ satisfying
    \begin{equation}
        \E[\CMKer_{\stepsize, l}^\circ]{ \norm{q^1 - q^2} \mid q_0^1, q_0^2 } \leq \lambda_2 \norm{q_0^1 - q_0^2}
        \label{eq:contractivity-ot}
    \end{equation}
    for all $(q_0^1, q_0^2) \in S \times S$,
    where $\CMKer_{\stepsize, l}^\circ$ is the coupled kernel in Algorithm~\ref{alg:coupled-hmc} with (i) shared momentum, (ii) shared forward and backward simulation steps and (iii) $(i, j) \sim \gamma^\circ$ for intra-trajectory sampling.
    \label{lemma:contractivity-ot}
\end{lemma}
\begin{proof}
    The definition of OT coupling in \eqref{eq:ot_objective} implies
    \begin{equation}
        \E[(i, j) \sim \gamma^\circ] { \norm{\flowqdisc{\stepsize{}}{l_i}(q_0^1, p_0) - \flowqdisc{\stepsize{}}{l_j}(q_0^2, p_0)} } \leq A_2.
    \end{equation}
    where $A_2$ is given in \eqref{eq:lemma-4.2-A2}.
    The rest of the proof follows exactly as that of Lemma~\ref{lemma:contractivity-maximal}.
\end{proof}
    Note that this implies the OT coupling has \emph{at least} as small contraction rate as the maximal coupling.

Finally, although the proof in this subsection relies on results from \citet{heng_unbiased_2019},
in particular Lemma 1 in \citet{heng_unbiased_2019},
we emphasize that the next section is not restricted to the special strategy of establishing local contractivity here.
In fact, any possible means of establishing local contractivity would work with the next section to establish geometric tails for relaxed meeting time,
which provides future opportunities to tighten the bound established here.

\subsection{Geometric tails via local contractivity}
\label{sec:theory-tails}

We now establish geometric tails of the relaxed meeting time using the local contractivity property of coupled HMC kernels we establish.
Our motivation to establish geometric tails in this specific manner is from the relation of multinomial coupled HMC to the OT formulation,
as it is already exploited in Section~\ref{sec:theory-local_contractivity-ot}.

We first restate the local contractivity property as an assumption to make our main theorem clean.
\begin{assumption}[Local contractivity]
    There exists a compact set $ S \in \calB(\RR) $, with positive Lebesgue measure,
    such that for a coupled HMC kernel $\CMKer$,
    there exists a contractivity rate $\lambda_0 \in (0, 1)$ satisfying
    \begin{equation}
        \E[\CMKer]{ \norm{q^1 - q^2} \mid q_0^1, q_0^2} \leq \lambda_0 \norm{q_0^1 - q_0^2}
    \end{equation}
    for any $(q_0^1, q_0^2) \in S \times S$.
    \label{ass:local_contractivity}
\end{assumption}

Similarly to Theorem 1 in \citet{heng_unbiased_2019},
our main theorem also assumes the existence of a global Lyapunov function for the corresponding HMC kernel,
which we state as a standalone assumption as below.
\begin{assumption}[Global Lyapunov function]
    For a Markov kernel $\MKer$,
    there exists a measurable function $V: \RR^d \mapsto [1, \infty)$, $\lambda \in (0, 1)$, $b < \infty$ such that
    \begin{equation}
        \E[\MKer]{ V(x) \mid x_0 } \leq \lambda V(x_0) + b
    \end{equation}
    for all $x \in \RR^d$ and $\E[x_0 \sim \pi_0]{ V(x_0)} < \infty$.
    $V$ is called the \textit{Lyapunov function}.
    \label{ass:global_lyapunov_function}
\end{assumption}

We now state our main theorem for geometric tails for the relaxed meeting time.
\begin{theorem}
    Suppose that there exists $\stepsize{}_0 > 0$ and $L_0 > 0$ such that for any $\stepsize{} \in (0, \stepsize{}_0)$ and $L > 0$ satisfying $\stepsize{} L < \stepsize{}_0 L_0$
    \begin{enumerate}
        \item The coupled HMC kernel $\CMKer_{\stepsize{},L}$ satisfies Assumption~\ref{ass:local_contractivity} on the compact set $ S \in \calB(\RR) $ with a contractivity rate $\lambda_0$, and
        \item Its marginal kernel $\MKer_{\stepsize{},L}$ satisfies Assumption~\ref{ass:global_lyapunov_function} with the Lyapunov function $V$ together with $\{ q_0 \in \RR^d : V(q) \leq \ell_1 \} \subseteq \{ q \in S : U(q) \leq \ell_0 \}$ for some $\ell_0 \in \{ \inf_{q\in S} U(q), \sup_{q\in S} U(q) \}$ and $\ell_1 > 1$ satisfying $\lambda + 2 b (1 + \ell_1)^{-1} < 1$.
    \end{enumerate}
    Then for any $\delta > 0$ and all $ n \in \NN$, we have
    \begin{equation}
        \pr_{\stepsize{}, L} (\tau_\delta > n) \leq C_0 \kappa^n
    \end{equation}
    for constant $C_0 \in \RR_+$ and $\kappa \in (0, 1)$.
    \label{theorem:geometric_tails}
\end{theorem}

\begin{remark}
    Although our proof strategy is different from \citet{heng_unbiased_2019},
    \thmref{theorem:geometric_tails} is consistent with Theorem 1 in \citet{heng_unbiased_2019} but replaces Proposition 1 in \citet{heng_unbiased_2019} with the local contractivity assumption.
    Also, the conditions stated right after \assumptref{ass:global_lyapunov_function} in \thmref{theorem:geometric_tails} is less strict compared
    to the corresponding assumption in Theorem 1 in \citet{heng_unbiased_2019}, 
    which is $ \lambda + 2 b \underline{(1 - \lambda)^{-1}} (1 + \ell_1)^{-1} < 1 $, where the extra term is underlined.
\end{remark}

\begin{proof}
    The proof is done by constructing a Lyapunov function that controls excursions outside of a set $\bar{C}_\delta \subseteq D_\delta$ by combining two Lyapunov functions induced by the two assumptions respectively.
    Once such Lyapunov function is obtained, 
    we can use the ``standard'' strategy used to prove the drift condition to establish the geometric tail.
    See Appendix~\ref{app:proof-geometric_tails} for the complete proof.
\end{proof}

Figure~\ref{fig:excursion} uses Venn diagrams to visualize how 
the global Lyapunov function and local contractivity 
are combined together to control excursions and establish geometric tails of relaxed meeting time.
\begin{figure}[t]
    \centering
\ffigbox[\textwidth]{%
    \begin{subfloatrow}[3]
        \ffigbox[0.25\textwidth]
        {\caption{Global}\label{fig:excursion-lyapunov}}
        {\scalebox{0.6}{\input{plots/proof/global_lyapunov_function}}}
        \ffigbox[0.25\textwidth]
        {\caption{Local}\label{fig:excursion-contractivity}}
        {\scalebox{0.6}{\input{plots/proof/local_contractivity}}}
        \ffigbox[0.25\textwidth]
        {\caption{Combined}\label{fig:excursion-combined}}
        {\scalebox{0.6}{\input{plots/proof/combined}}}
    \end{subfloatrow}
}{%
    \caption{Controlling excursions outside of sets. In Figure~\ref{fig:excursion-lyapunov}, the time of entering the unshaded set is geometrically fast but that set is not what we target for meeting. In Figure~\ref{fig:excursion-contractivity}, the unshaded set is the target set but there is not a valid Lyapunov function to control excursion. In Figure~\ref{fig:excursion-combined}, the intersection of previous two unshaded set is equipped with a valid Lyapunov function and corresponds to relaxed meeting.
    Entering this set $\bar{C}_\delta$ geometrically fast is shown in the proof of Theorem~\ref{theorem:geometric_tails}.}
    \label{fig:excursion}
}
\end{figure}

Together with Lemma~\ref{lemma:contractivity-maximal}, Lemma~\ref{lemma:contractivity-ot},
Theorem~\ref{theorem:geometric_tails} proves that coupled multinomial HMC with maximal coupling and OT coupling has geometric tails for its relaxed meeting time,
which is the sufficient condition to satisfy Assumption~\ref{ass:tail_of_meeting_time} and Assumption~\ref{ass:faithfullness} in order to use the unbiased estiamtes in \eqref{eq:H_k} and \eqref{eq:H_km}.

